Verification and Control of Partially Observable Probabilistic Real-Time Systems

We propose automated techniques for the verification and control of probabilistic real-time systems that are only partially observable. To formally model such systems, we define an extension of probabilistic timed automata in which local states are partially visible to an observer or controller. We give a probabilistic temporal logic that can express a range of quantitative properties of these models, relating to the probability of an event's occurrence or the expected value of a reward measure. We then propose techniques to either verify that such a property holds or to synthesise a controller for the model which makes it true. Our approach is based on an integer discretisation of the model's dense-time behaviour and a grid-based abstraction of the uncountable belief space induced by partial observability. The latter is necessarily approximate since the underlying problem is undecidable, however we show how both lower and upper bounds on numerical results can be generated. We illustrate the effectiveness of the approach by implementing it in the PRISM model checker and applying it to several case studies, from the domains of computer security and task scheduling.

==> appx-approx.tex <==
\section{Approximate solution}

\subsection*{Approximation scheme}

we first  define the value function for expected (reward) reachability \todo{add in the target states (which have value 0)}
\begin{align}
\lefteqn{V(b) \;= \; \left\{ 
\begin{array}{cl}
0 & \mbox{if $b$ in target} \\
\min_{a \in A} \left\{ R(b,a) + \sum_{b' \in \dist(S)} P[ \, b' \, | \, a,b \, ] {\cdot} V(b') \right\} & \mbox{otherwise}
\end{array} \right.} \nonumber \\
& = \; \min_{a \in A} \left\{ R(b,a) + \sum_{b' \in \dist(S)} \sum_{o \in O} \mathrm{Pr}[ \, b' \, | \, o,a,b \, ] {\cdot} \mathrm{Pr}[ \, o \, | \, a,b \, ] {\cdot} V(b') \right\} & \mbox{using \eqnref{belieftrans-eqn}} \nonumber\\
& = \; \min_{a \in A} \left\{ R(b,a) + \sum_{o \in O}  \mathrm{Pr}[ \, o \, | \, a,b \, ] {\cdot} \left( \sum_{b' \in \dist(S)} \mathrm{Pr}[ \, b' \, | \, o,a,b \, ] {\cdot} V(b') \right) \right\} & \mbox{rearranging} \nonumber \\
& = \; \min_{a \in A} \left\{ R(b,a) + \sum_{o \in O} \mathrm{Pr}[ \, o \, | \, a,b \, ] {\cdot} V(b^{a,o}) \right\} & \mbox{by definition of $b^{a,o}$.} \label{value-eqn}
\end{align}
Note: probabilistic reachability is similar - the reward $R(b,a)$ is omitted and the targets have value 1 rather than 0.

An approximation scheme for the belief MDP is:
\begin{itemize}
\item
a finite set of beliefs $G = \{ g_1 , \dots , g_K \}$ where the convex hull of $G$ is $\dist(S)$;
\item
a representation scheme $\underline{\gamma} : \dist(S) \rightarrow \Rset^K$, such that for any belief $b$ we have 
\[
b = \sum_{j=1}^{K} \gamma_j(b) \cdot g_j \,.
\]  
\end{itemize}
From \eqnref{value-eqn}, the Bellman equation for expected (reward) reachability over the belief MDP (ignoring the targets) is such that for any belief $b$ we have:
\[
V(b) = \min_{a \in A} \left\{ R(b,a) + \sum_{o \in O} P[ \, o \, | \, a,b \, ] \cdot V(b^{a,o}) \right\}
\]
Let us now consider computing $V(b)$ over the finite set of beliefs $G = \{ g_1 , \dots , g_K \}$. Now both $A$ and $O$ are finite sets, $R(b,a)$ can be computed using \eqnref{beliefreward-eqn} and the reward function of the POMDP and $P[ \, o \, | \, a,b \, ]$, the probability of observing $o$ given we were in belief $b$ and performed action $a$, can be computed as shown in \eqnref{oba-eqn} using the transition and observation functions of the POMDP. However, considering $V(b^{a,o})$ since the belief $b^{a,o}$ is not necessarily a member of $G$ even if $b$ is (recall $b^{a,o}$ is the belief we end up in if we perform action $a$ and observe $o$ from belief $b$).
\\ \\
This is where the representation scheme comes in, by construction we have $b^{a,o} = \sum_{j=1}^k \gamma_j(b^{a,o})\cdot g_j$, so instead we can approximate $V(b^{a,o})$ with the value:
\[
\sum_{j=1}^K \gamma_j(b^{a,o}) \cdot V(g_j) \, .
\]
which is now over $G$. Assuming the representation function is computable, for any $b \in G$ we:
\begin{enumerate}
\item
use \eqnref{bao-eqn} to calculate the belief $b^{a,o}$;
\item then use the representation function to compute $\gamma_j(b^{a,o})$ for each $1 \leq j \leq K$.
\end{enumerate}
From the results of Yu and Bertsekas \cite{YB04} using this approximation will lead to a \emph{lower bound} on the actual result. In addition, \cite{Yu06} states that this is the approximation scheme proposed by \cite{ZH01} for discounted problems.
\\ \\
More precisely (ignoring targets), the approximate value iteration scheme is such that for any $g_i \in G$:
\begin{equation}\label{j1-eqn}
\tilde{V}_{n+1}(g_i) = \min_{a \in A} \left\{ R(g_i,a) + \sum_{o \in O} P[ \, o \, | \, a,g_i \, ] \cdot \left( \sum_{j=1}^k \gamma_j(g_i^{a,o}) \cdot \tilde{V}_n(g_j) \right) \right\}
\end{equation}
Notice that a number of these terms remain fixed during each iteration so can be computed once at the start
\gethin{mention \cite{SPK13} for optimisations?}
\gethin{initial approximation (maybe used the values obtained on the POMDP when everything is observable?} \\ \\
In \cite{YB04} and \cite{Yu06} there is an alternative representation scheme which corresponds to apply the representation scheme to the current belief rather than the belief after an action and observation. Taking this approach, rather than considering values for the finite set of beliefs $G$, the values we compute are for beliefs of the form $g_j^{a,o}$, more precisely the approximation is being performed over the finite set of beliefs $\{ g_j^{a,o} \, | \, 1 {\leq} j {\leq} K \wedge a \in A \wedge o\in O \}$ and the approximate value iteration scheme is given by:
\begin{equation}\label{j2-eqn}
\tilde{V}_{n+1}(b) = \min_{a \in A} \left\{ R(b,a) + \sum_{j=1}^k \gamma_j(g_i) \cdot \left( \sum_{o \in O}  \cdot P[ \, o \, | \, a,g_j \, ] \cdot \tilde{V}_n(g_j^{a,o}) \right)  \right\}
\end{equation}

\subsection*{Fix resolution grid (Lovejoy \cite{Lov91})}
We now define the regular grid construction of Lovejoy \cite{Lov91}. We assume that the POMDP has a state space of size $N$. \\ \\
Let $M$ be a positive integer that represents the \emph{resolution} of the grid. The set of grid points (belief states) is defined as:\footnote{I am assuming $\Nset$ includes 0.}
\[
G = \left\{ \frac{1}{M} v  \, \left| \, v \in \Nset^{N} \wedge \sum_{i=1}^N v(i) {=} M  \right. \right\}
\]
The number of grid points $K$ is given by the following formula:
\[
\frac{(M + N -1)!}{M! ( N-1)!}
\]
Following Lovejoy \cite{Lov91}, we now give a method for computing the representation function. More precisely, given an arbitrary belief $b$ we need to compute $\lambda_j$ for $1\leq j \leq K$ such that
\[
b = \sum_{j=1}^{K} \lambda_j \cdot g_j
\]
Note that the values $\lambda_j$ are not unique. The approach of \cite{Lov91} is based on finding the smallest sub-simplex that contains $b$ and then finding the coefficients $\lambda_j$ for the elements of this sub-simplex (for elements outside the subsimplex $\lambda_j$ will be 0). To do this the following second grid of (integer) vectors is used:
\[
G' = \left\{ q \in \Nset^{N}  \, \left| \, M = q(1) \geq q(2) \geq \cdots \geq q(N) \geq 0   \right. \right\}
\]
The construction is based on first converting $b$ into a vector $q \in G'$. Then, since there is a one-to-one relationship between $G$ and $G'$, the sub-simplex that contains $q \in G'$ can be used to determine the subsimplex of $G$ that contains $b$. Given an element $q$ of $G'$ the corresponding element of $G$ is given by:
\begin{equation}\label{primetog-eqn}
\frac{1}{M}(q(1){-}q(2),q(2){-}q(3),\dots,q(n{-}1){-}q(n),q(n)) \, .
\end{equation}
Note by definition of $G'$ we have $q(1)$ equals $M$.
On the other hand given an element $g$ of $G$, the corresponding element of $G'$ is constructed as follows:
\begin{equation}\label{gtoprime-eqn}
\begin{array}{c}
M \left(\sum_{j=1}^N g(j) ,\sum_{j=2}^N g(j),\dots,\sum_{j=N-1}^N g(j),\sum_{j=N}^N g(j) \right)
\end{array}
\end{equation}
We now summarises the steps of \cite{Lov91} for constructing the representation of a belief $b$ as given in \cite{ZH01}. We suppose there is an enumeration of the state space $S = \{ s_1, \dots , s_N \}$.
\begin{enumerate}
\item
create $x$ where $x(i) = M {\cdot} \sum_{j=i}^N b(i)$. (This transforms $b$ from a pdf to a cdf. This is not in $G'$ as the values of $x$ need not be integers, i.e. when $b$ is not in $G$. However it does correspond to the mapping used to go from elements of $G$ to elements of $G'$ given in \eqnref{gtoprime-eqn}.)
\item
let $v$ be the largest integer vector such that $v(i) \leq x(i)$ for $1 \leq i \leq N$. (Essentially just taking the floor of all values in $x$. This gives an element in $G$ as $x(1)$ will by construction equal 1.)
\item
let $d$ be the vector where $d(i) = x(i) {-} v(i)$ for $1 \leq i \leq N$. (These are the fractional differences so will need to be encoded in the $\lambda_i$'s as the grid point of $G'$ take only integer values. So the remainder should explain how to do this.)
\item
let $p : \{1,\dots,N\} \rightarrow \{1,\dots,N\}$ be a permutation of $1,\dots,N$ such that after the permutation the elements of $d$ are in decending order, i.e.\ we have $d(p(1)) \geq d(p(2)) \geq \cdots \geq d(p(N))$. (In \cite{Lov91} it states that any permutation will work so there is no need to choose a specific permutation when it is not unique.)
\item 
we now find integer vectors $v_1,\dots,v_N$ which can then be used to build a sub-simplex of $G'$ containing $x$. More precisely we let:
\begin{align*}
v_1 & = \; v  \\
v_{i+1} & = v_i + e_{p(i)} & \mbox{for $2 \leq i \leq N-1$}
\end{align*}
where $e_{i}$ is the $i$th unit vector. (This is called the \emph{Freudenthal triangulation} \cite{Eav84}. It is possible some of the vectors created will not be in $G'$, however for any such vectors the corresponding coordinates constructed below will be zero so these vectors can be ignored \cite{Lov91}.) 
\item Using \eqnref{primetog-eqn}, map the elements $v_1,\dots,v_N$ to elements $q_1,\dots,q_N$ of $G$ which are a sub-simplex for $b$. (Recall the mapping \eqnref{primetog-eqn} was used to construct $x$ from $b$. In addition, as mentioned in 5 there may exist $1 \leq i \leq N$ such that $v_i \not\in G'$, however these vectors can be ignored as the corresponding coordinate ($\lambda_i$) constructed in 6 will be zero).
\item Now we find the coordinates $\lambda_1 , \dots , \lambda_N$ such that $b = \sum_{i=1}^N \lambda_i g_i$ by setting:
\begin{align*}
\lambda_i & = \; d(p(i{-}1)) - d(p(i)) \; \; \mbox{for $2 \leq i \leq N$} \\
\lambda_1 & = \; 1 - \sum_{j=2}^N \lambda_j
\end{align*}
\end{enumerate}

\subsection*{Implementation in PRISM}
A PRISM model for a POMDP will include a list of the variables that are observable. Therefore, we can split the variables into those that are observable and those that are not, i.e. sets of variables $U_O$ and $V_{U}$. If we now consider a belief, since the observable variables can always be distinguished, in any belief state we will know the precise value of each observable variable (with probability 1). This therefore leads to a simpler notion of a belief state: assuming the observable and unobservable variables are $U_O = \{ u_1,\dots,u_{m}\}$ and $V_{U} =\{ v_1,\dots,v_{n} \}$, a belief state is a pair $(s_O,b_U)$ where:
\begin{itemize}
\item
$s_O$ is a valuation of each observable variable, i.e. a vector $s_O = (x_1,\dots,x_{m})$ where $x_i$ is the value of the observable variable $u_i$;
\item
$b_U$ is a distribution of the valuations of the unobservable variables, i.e. for any vector $s_U = (x_1,\dots,x_{m})$ of values of unobservable variables, we have $b_U(s_U)$ is the probability we belief the unobservable variables take the values in $s_U$.
\end{itemize}
Regarding the grid this will now be of the form
\[
G = \left\{ (s_O, \frac{1}{M} v)  \, \left| \, s_O \in S_O \wedge v \in \Nset^{N} \wedge \sum_{i=1}^N v(i) {=} M  \right. \right\}
\]
where $S_O$ is the set of all valuations of observable variables and $N$ is the number of valuations of unobservable variables. This should simplify the implementation as we now only considering distributions over a smaller number of states which will improve the efficiency of the steps of Lovejoy in the previous section.


